L2R-CIPU: Efficient CNN Computation with Left-to-Right Composite Inner Product Units

This paper proposes a composite inner-product computation unit based on left-to-right (LR) arithmetic for the acceleration of convolution neural networks (CNN) on hardware. The efficacy of the proposed L2R-CIPU method has been shown on the VGG-16 network, and assessment is done on various performance metrics. The L2R-CIPU design achieves 1.06x to 6.22x greater performance, 4.8x to 15x more TOPS/W, and 4.51x to 53.45x higher TOPS/mm2 than prior architectures.

==> Background/Background.tex <==
\section{Background}
\label{sec:Background}
%%
%%

==> Conclusion/Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion-future}
%%
Write you conclusion here...

==> Introduction/Introduction.tex <==
\section{Introduction}
\label{sec:Introduction}


